The Born rule as structure of spectral bundles (extended abstract)

Topos approaches to quantum foundations are described in a unified way by means of spectral bundles, where the base space is a space of contexts and each fibre is its spectrum. Differences in variance are due to the bundle being a fibration or opfibration. Relative to this structure, the probabilistic predictions of the Born rule in finite dimensional settings are then described as a section of a bundle of valuations. The construction uses in an essential way the geometric nature of the valuation locale monad.

==> eptcsdata.tex <==
\providecommand{\firstpage}{81}
\providecommand{\publicationstatus}{Bart Jacobs, Peter Selinger, and Bas Spitters (Eds.):\\ 8th International Workshop on Quantum Physics and Logic (QPL 2011)\\
EPTCS 95, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.95.8}{10.4204/EPTCS.95.8}}

